Geometric Shaping of 2-Dimensional Constellations in the Presence of Laser Phase Noise

In this paper, we propose a geometric shaping (GS) strategy to design 8, 16, 32 and 64-ary modulation formats for the optical fibre channel impaired by both additive white Gaussian (AWGN) and phase noise. The constellations were optimised to maximise generalised mutual information (GMI) using a mismatched channel model. The presented formats demonstrate an enhanced signal-to-noise ratio (SNR) tolerance in high phase noise regimes when compared with their quadrature amplitude modulation (QAM) or AWGN-optimised counterparts. By putting the optimisation results in the context of the 400ZR implementation agreement, we show that GS alone can either relax the laser linewidth (LW) or carrier phase estimation (CPE) requirements of 400 Gbit/s transmission links and beyond. Following the GMI validation, the performance of the presented formats was examined in terms of post forward error correction (FEC) bit-error-rate (BER) for a soft decision (SD) extended Hamming code (128, 120), implemented as per the 400ZR implementation agreement. We demonstrate gains of up to 1.2 dB when compared to the 64-ary AWGN shaped formats.

==> figures/cfec_model.tex <==
\begin{figure}[t]
\centering
\begin{minipage}{\columnwidth}
    \centering
    \scalebox{1.0}{
    \includegraphics[width=0.9\columnwidth]{pdf/cfec_encdec_cropped.pdf}}\hfill
\end{minipage}%
\caption{Combined FEC model suggestion - simplified.}
\label{fig:cfec_model}
\vspace{-12pt}
\end{figure}

==> figures/curves_16.tex <==
\begin{figure}[t]
        \centering
        \begin{minipage}{0.24\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{16QAM/Curves/GMI_1MHz.tikz}}
        \end{minipage}%
        \begin{minipage}{0.24\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{16QAM/Curves/GMI_2MHz.tikz}}\hfill
        \end{minipage}%
        \centering
        \vspace{.1cm}
        \begin{minipage}{0.24\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{16QAM/Curves/GMI_4MHz.tikz}}
        \end{minipage}%
        % \begin{minipage}{0.24\textwidth}
        %     \centering
        %     \scalebox{.93}{
        %     \includegraphics[width=\textwidth]{16QAM/Curves/dSNR.tikz}}\hfill
        % \end{minipage}%
        %
         \caption{GMI for 60~Gbaud, 16-\textit{ary} constellations assuming (a) a 1~MHz, (b) a 2~MHz and (c) a 4~MHz combined laser linewidths.}
        \label{fig:curves_16}
        \vspace{-12pt}
\end{figure}

==> figures/curves_32.tex <==
\begin{figure}[ht]
        \centering
        \begin{minipage}{0.24\textwidth}
            \centering
          \scalebox{.97}{
            \includegraphics[width=\textwidth]{32QAM/Curves/GMI_1MHz.tikz}}
        \end{minipage}%
        \begin{minipage}{0.24\textwidth}
            \centering
            \scalebox{.97}{
            \includegraphics[width=\textwidth]{32QAM/Curves/GMI_2MHz.tikz}}\hfill
        \end{minipage}%
        \centering
        \vspace{.1cm}
        \begin{minipage}{0.24\textwidth}
            \centering
            \scalebox{.97}{
            \includegraphics[width=\textwidth]{32QAM/Curves/GMI_4MHz.tikz}}
        \end{minipage}%
        % \begin{minipage}{0.24\textwidth}
        %     \centering
        %     \scalebox{.93}{
        %     \includegraphics[width=\textwidth]{32QAM/Curves/dSNR.tikz}}\hfill
        % \end{minipage}%
        %
         \caption{GMI  60~Gbaud, 32-\textit{ary} constellations assuming (a) a 1~MHz, (b) a 2~MHz and (c) a 4~MHz combined laser linewidths.}
        \label{fig:curves_32}
        \vspace{-12pt}
\end{figure}

==> figures/curves_64.tex <==
\begin{figure}[b]
        \centering
        \begin{minipage}{0.24\textwidth}
            \centering
          \scalebox{.97}{
            \includegraphics[width=\textwidth]{64QAM/Curves/GMI_1MHz.tikz}}
        \end{minipage}%
        \begin{minipage}{0.24\textwidth}
            \centering
            \scalebox{.97}{
            \includegraphics[width=\textwidth]{64QAM/Curves/GMI_2MHz.tikz}}\hfill
        \end{minipage}%
        \centering
        \vspace{.1cm}
        \begin{minipage}{0.24\textwidth}
            \centering
            \scalebox{.97}{
            \includegraphics[width=\textwidth]{64QAM/Curves/GMI_4MHz.tikz}}
        \end{minipage}%
        % \begin{minipage}{0.24\textwidth}
        %     \centering
        %     \scalebox{.93}{
        %     \includegraphics[width=\textwidth]{64QAM/Curves/dSNR.tikz}}\hfill
        % \end{minipage}%
        %
         \caption{GMI for 60~Gbaud, 64-\textit{ary} constellations assuming (a) a 1~MHz, (b) a 2~MHz and (c) a 4~MHz combined laser linewidths.}
        \label{fig:curves_64}
        \vspace{-12pt}
\end{figure}

==> figures/curves_8.tex <==
\begin{figure}[t]
        \centering
        \begin{minipage}{0.24\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{8QAM/Curves/GMI_1MHz.tikz}} 
        \end{minipage}%
        \begin{minipage}{0.24\textwidth}
            \centering
             \scalebox{.96}{
            \includegraphics[width=\textwidth]{8QAM/Curves/GMI_2MHz.tikz}}\hfill
        \end{minipage}%
        \centering
        \vspace{.1cm}
        \begin{minipage}{0.24\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{8QAM/Curves/GMI_4MHz.tikz}}
        \end{minipage}%
        % \begin{minipage}{0.24\textwidth}
        %     \centering
        %     \scalebox{.93}{
        %     \includegraphics[width=\textwidth]{8QAM/Curves/dSNR.tikz}}\hfill
        % \end{minipage}%
        %
        \caption{GMI for 60~Gbaud, 8-\textit{ary} constellations assuming (a) a 1~MHz, (b) a 2~MHz and (c) a 4~MHz combined laser linewidths.}
        \label{fig:curves_8}
        \vspace{-12pt}
\end{figure}

==> figures/fec_curves_16.tex <==
\begin{figure}[t]
        \centering
        \begin{minipage}{0.23\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{16QAM/Curves/SD_Hamming_M=16_RPN=1.0e-04.tikz}} 
        \end{minipage}%
        \begin{minipage}{0.23\textwidth}
            \centering
             \scalebox{.96}{
            \includegraphics[width=\textwidth]{16QAM/Curves/SD_Hamming_M=16_RPN=2.1e-04.tikz}}\hfill
        \end{minipage}%
        \centering
        \vspace{.1cm}
        \begin{minipage}{0.23\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{16QAM/Curves/SD_Hamming_M=16_RPN=4.2e-04.tikz}}
        \end{minipage}%
        % \begin{minipage}{0.23\textwidth}
        %     \centering
        %     \scalebox{.93}{
        %     \includegraphics[width=\textwidth]{16QAM/Curves/dSNR_fec.tikz}}\hfill
        % \end{minipage}%
        %
        \caption{SD Hamming(128, 120) post-FEC performance for 60~Gbaud, 16-\textit{ary} constellations assuming (a) a 1~MHz, (b) a 2~MHz and (c) a 4~MHz combined laser linewidths. (d) SNR penalty vs. phase noise variance at the post-FEC threshold of $4.5\cdot 10^{-3}$..}
        \label{fig:fec_curves_16}
        \vspace{-12pt}
\end{figure}

==> figures/fec_curves_32.tex <==
\begin{figure}[t]
        \centering
        \begin{minipage}{0.23\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{32QAM/Curves/SD_Hamming_M=32_RPN=1.0e-04.tikz}} 
        \end{minipage}%
        \begin{minipage}{0.23\textwidth}
            \centering
             \scalebox{.96}{
            \includegraphics[width=\textwidth]{32QAM/Curves/SD_Hamming_M=32_RPN=2.1e-04.tikz}}\hfill
        \end{minipage}%
        \centering
        \vspace{.1cm}
        \begin{minipage}{0.23\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{32QAM/Curves/SD_Hamming_M=32_RPN=4.2e-04.tikz}}
        \end{minipage}%
        % \begin{minipage}{0.23\textwidth}
        %     \centering
        %     \scalebox{.93}{
        %     \includegraphics[width=\textwidth]{32QAM/Curves/dSNR_fec.tikz}}\hfill
        % \end{minipage}%
        %
        \caption{SD Hamming(128, 120) post-FEC performance for 60~Gbaud, 32-\textit{ary} constellations assuming (a) a 1~MHz, (b) a 2~MHz and (c) a 4~MHz combined laser linewidths. (d) SNR penalty vs. phase noise variance at the post-FEC threshold of $4.5\cdot 10^{-3}$.}
        \label{fig:fec_curves_32}
        % \vspace{-12pt}
\end{figure}

==> figures/fec_curves_64.tex <==
\begin{figure}[t]
        \centering
        \begin{minipage}{0.23\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{64QAM/Curves/SD_Hamming_M=64_RPN=1.0e-04.tikz}} 
        \end{minipage}%
        \begin{minipage}{0.23\textwidth}
            \centering
             \scalebox{.96}{
            \includegraphics[width=\textwidth]{64QAM/Curves/SD_Hamming_M=64_RPN=2.1e-04.tikz}}\hfill
        \end{minipage}%
        \centering
        \vspace{.1cm}
        \begin{minipage}{0.23\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{64QAM/Curves/SD_Hamming_M=64_RPN=4.2e-04.tikz}}
        \end{minipage}%
        % \begin{minipage}{0.23\textwidth}
        %     \centering
        %     \scalebox{.93}{
        %     \includegraphics[width=\textwidth]{64QAM/Curves/dSNR_fec.tikz}}\hfill
        % \end{minipage}%
        %
        \caption{SD Hamming(128, 120) post-FEC performance for 60~Gbaud, 64-\textit{ary} constellations assuming (a) a 1~MHz, (b) a 2~MHz and (c) a 4~MHz combined laser linewidths. (d) SNR penalty vs. phase noise variance at the post-FEC threshold of $4.5\cdot 10^{-3}$.}
        \label{fig:fec_curves_64}
        \vspace{-12pt}
\end{figure}

==> figures/fec_curves_8.tex <==
\begin{figure}[t]
        \centering
        \begin{minipage}{0.23\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{8QAM/Curves/SD_Hamming_M=8_RPN=1.0e-04.tikz}} 
        \end{minipage}%
        \begin{minipage}{0.23\textwidth}
            \centering
             \scalebox{.96}{
            \includegraphics[width=\textwidth]{8QAM/Curves/SD_Hamming_M=8_RPN=2.1e-04.tikz}}\hfill
        \end{minipage}%
        \centering
        \vspace{.1cm}
        \begin{minipage}{0.23\textwidth}
            \centering
            \scalebox{.96}{
            \includegraphics[width=\textwidth]{8QAM/Curves/SD_Hamming_M=8_RPN=4.2e-04.tikz}}
        \end{minipage}%
        % \begin{minipage}{0.23\textwidth}
        %     \centering
        %     \scalebox{.93}{
        %     \includegraphics[width=\textwidth]{8QAM/Curves/dSNR_fec.tikz}}\hfill
        % \end{minipage}%
        %
        \caption{SD Hamming(128, 120) post-FEC performance for 60~Gbaud, 8-\textit{ary} constellations assuming (a) a 1~MHz, (b) a 2~MHz and (c) a 4~MHz combined laser linewidths. (d) SNR penalty vs. phase noise variance at the post-FEC threshold of $4.5\cdot 10^{-3}$.}
        \label{fig:fec_curves_8}
        \vspace{-12pt}
\end{figure}

==> figures/fec_verification.tex <==
\begin{figure*}[h]
        \centering
        \begin{minipage}{0.25\textwidth}
            \centering
            \scalebox{.97}{
            \includegraphics[width=\textwidth]{16QAM/ber_mismatched.tikz}}
        \end{minipage}%
        \begin{minipage}{0.25\textwidth}
            \centering
            \scalebox{.97}{
            \includegraphics[width=\textwidth]{16QAM/ber_mismatched.tikz}}
        \end{minipage}%
        \begin{minipage}{0.25\textwidth}
            \centering
            \scalebox{.97}{
            \includegraphics[width=\textwidth]{16QAM/ber_mismatched.tikz}}
        \end{minipage}%
        %
        \centering
        \vspace{5mm}
        \begin{minipage}{0.25\textwidth}
            \centering
            \scalebox{.97}{
            \includegraphics[width=\textwidth]{16QAM/ber_matched.tikz}}
        \end{minipage}%
        \begin{minipage}{0.25\textwidth}
            \centering
            \scalebox{.97}{
            \includegraphics[width=\textwidth]{16QAM/ber_matched.tikz}}
        \end{minipage}%
        \begin{minipage}{0.25\textwidth}
            \centering
            \scalebox{.97}{
            \includegraphics[width=\textwidth]{16QAM/ber_matched.tikz}}
        \end{minipage}%
        %
        \caption{Phase noise shaped constellations for: (a) 500kHz mismatched, (b) 500kHz matched, (c) 1MHz mismatched and (d) 1MHz matched receiver models. The binary bit to symbol mapping is presented as hexadecimal numbers.}
        \label{fig:fec_verif}
\end{figure*}

==> sections/X_old_II_Background.tex <==
\section{An overview of geometric shaping in presence of phase noise}
\label{sec:shaping}
\raggedbottom
%
% Channel model and phase noise modelling 
Consider a discrete-time channel which at any given time instant can be described as
%
\begin{equation}
\label{eq:chm}
Y = X \cdot e^{j\phi_n} + \mathcal{N}
\end{equation}
% 
,where $X$ is a random variable representing the transmitted symbol, $\mathcal{N}$ represents a complex zero-mean Gaussian random variable and Y is the received symbol. Each symbol $X$ is selected from the complex constellation $\mathcal{C} =\left[C_{1}, C_{2}, \ldots, C_{M}\right]$ of a size $M$, whereas $\phi_n$ is a of random Gaussian variables with a variance modelled as
%
\begin{equation}
\sigma^2_{\text{RPN}}=2\pi\Delta\nu\Delta{T_{S}}
\end{equation}
%
where $\Delta{T}_{S}$ denotes symbol time and $\Delta\nu$ is a combined linewdith of the LO and laser. It should be highlighted that the constellations are optimised for the RPN remaining after the CPE.  Therefore, random walk component is assumed to be compensated for at this stage. 

Given a BICM system supported with a binary SD-FEC code, the detection process can be split into two stages: first, a bit-wise demapper calculates ``soft" information about the bits (expressed as LLs); subsequently, its output is passed to a binary SD-FEC decoder. The resulting system model is shown in Fig. \ref{fig:system_model}.
% Figure with BICM binary SD-FEC encoder-decoder pair with the appropriate caption goes hereeeee. 
\input{figures/constellations_16.tex}
\input{figures/constellations_32.tex}
% Achievable information rates 
\subsection{Performance metrics}
Although it is possible to design a modulation format for a specific FEC, it would require individual adjustment for each code. Conveniently, information-theoretic metrics, under the assumption of BICM, allow the approximation of the system performance for any FEC. Considering a non-binary SD-FEC encoder-decoder pair, MI is the most popular performance predictor \cite{Schmalen2017}. For any memoryless optical fibre channel, it can be formulated as
%
\begin{equation}
\mathrm{MI}=I(\boldsymbol{X} ; \boldsymbol{Y}) \triangleq \mathbb{E}\left[\log _{2} \frac{f_{\boldsymbol{Y} | \boldsymbol{X}}(\boldsymbol{Y} | \boldsymbol{X})}{f_{Y}(\boldsymbol{Y})}\right]
\end{equation}
%
where $X$ stands for the input, $Y$ represents the output symbols, $\mathbb{E}$ is the expectation and $f_{\boldsymbol{Y} | \boldsymbol{X}}$ denotes the channel law. In case of binary SD-FEC codes, the performance can be approximated with GMI \cite{Alvarado2016}. It represents a bit-wise sum of $m = \log_2(M)$ MIs with $M$ being the constellation order. The GMI is defined as 
%
\begin{equation}
\mathrm{GMI} \triangleq \sum_{i=1}^{m} I\left(B_{i} ; \boldsymbol{Y}\right)=\sum_{i=1}^{m} \mathbb{E}\left[\log _{2} \frac{f_{Y | B_{i}}\left(\boldsymbol{Y} | B_{i}\right)}{f_{Y}(\boldsymbol{Y})}\right]
\end{equation}
%
where $[B_{1}, B_{2}, \ldots, B_{m}]$ is a bit-wise representation of the channel input, assuming that each symbol $X$ represented with the $m$ number of bits. The third performance metric is SER, also called pre-FEC threshold. It is used to predict the minimum SNR threshold needed for the error-free recovery of an ideal binary nonbinary HD FEC code \cite{Liga_2017}. In this work, we will focus on SD-FEC performance for a binary FEC code, thus optimise the modulation formats to maximise the GMI. 
% Mismatched receiver model
\input{figures/constellations_64.tex}
\subsection{Mismatched receiver model}
Under the assumption of an ideal transmission model, the receiver determines the averaged probability density function (PDF) of the channel to calculate the soft information about the recovered data. Nevertheless, it is often non-trivial to approximate the channel function or computationally expensive to calculate the log-likelihood ratios (LLRs) concerning a matched model \cite{Schmalen2017}. Therefore, a more common approach is to use a mismatched receiver\cite{Merhav_1994}, given by 
\begin{equation}
f_{Y_{n} | \mathbf{X}_{n}}(\boldsymbol{y} | \boldsymbol{x})=\frac{1}{\left(\pi N_{0}\right)^{2}} \exp \left(-\frac{\|\boldsymbol{y}-\boldsymbol{x}\|^{2}}{N_{0}}\right)
\end{equation}
where $X_{n}$ and $Y_{n}$ are 2-dimensional (2D) complex symbols, $N_{0}$ is a 2D variance of an independent, zero-mean, random Gaussian variable vector and the $||y  - x||^2$ denotes a squared Euclidean distance between the symbols.  

% Matched receiver model
\subsection{PCAWGN auxiliary channel model}
Alternatively, it is possible to consider both linear and angular components of the received signal after conditioning with sufficient digital signal processing (DSP) techniques \cite{Savory2010}. As mentioned in Section \ref{sec:shaping}, the PCAWGN was addressed in several studies \cite{Hou_2003, Goebel_2011, Foschini_AWGNPN_1973}. Recently, the work in \cite{Sales_2019} proposed a reduced-complexity PCAWGN approximation, given by
%
\begin{equation}
\begin{array}{c}{
{f_{Y_{n}| X_{n}} (\boldsymbol{y} | \boldsymbol{x}) \approx \frac{K}{\pi \gamma N_{0}} \exp \left(-\frac{\Delta \rho^{2}+(\gamma \Delta \theta)^{2}}{N_{0}}\right)}} \\
\\
{\gamma=\left(\frac{1}{|x| \rho}+\frac{2}{\alpha N_{0}}\right)^{-\frac{1}{2}}}
\end{array}
\end{equation}
where $X_{n}$ and $Y_{n}$ are 2-dimensional (2D) complex symbols, $\alpha \approx \frac{1}{\sigma_{2}}$ is used to model the phase noise with a variance $\sigma^{2}$. Consequently, the $N_{0}$ is a 2D variance of an independent, zero-mean, random Gaussian variable vector and $K \approx 1$ for high SNR. The other components, described as 
\begin{equation}
\begin{array}{c}{
{\Delta \rho=\rho-|x|}} \\ 
\\
\Delta \theta=\arg(y)-\arg (x), \quad \Delta \theta \in[-\pi, \pi)
\end{array}
\end{equation}
%
are subsequently: the Euclidean distance $\Delta \rho$ between the received and the expected symbol, represented as $\rho$ and $x$ respectively; the angular difference $\Delta \theta$ between $x$ and $y$. Moreover, the presented PCAWGN model also reduces the information loss (measured with AIRs) compared to the other metrics.  

% Optimisation algorithm
\subsection{Constellation optimisation}
Under the assumption of a binary SD-FEC encoder-decoder pair, all of the demonstrated constellations were optimised to maximise the GMI performance. The presented GS strategy is based on the first stage of the gradient descent algorithm proposed in \cite{Schrekenbach_2013}, combined with a binary label switching method from \cite{Chen_2018_GS64} to optimise bit-to-symbol mapping. It should be noted that the demonstrated approach does not guarantee to find the global optima. However, the resulting constellations outperformed the corresponding M-QAM formats.

The AWGN shaped constellations were optimised using Gauss-Hermite numerical integration formula from \cite{salzer_1952}. Considering the channel model presented in Eq. (\ref{eq:chm}), the $\phi_n$ component was set as a zero-valued vector, hence disabled the phase noise impairments. Subsequently, the resulting AWGN shaped constellations were used to initialise the AWGN+PN optimiser based on the Monte-Carlo methodology with $2^{19}$ randomly interleaved symbols per iteration. In that case, the GMI performance of all presented modulation formats depend on both AWGN and phase noise components.Therefore, 8- , 16-, 32-, 64-\textit{ary} constellations were optimised over a range of SNR and RPN values for each receiver model.
%
% Verification procedure 
\subsection{Verification of the shaping results}
The performance of both AWGN and AWGN+PN constellations was examined in a simulated Monte Carlo channel with both AWGN and a ``random walk'' phase noise impairments. Each combination of the AWGN and phase noise values was verified using $2^{20}$ symbols per iteration. The CPE was undertaken with a format-agnostic recovery scheme \cite{Mazur_19, Yuta_2019}, where the QPSK pilots were inserted between every 32 data symbols. Then, the estimated phase information was interpolated over the entire data frame using Wiener filter coefficients calculated from \cite{Ip_2007}. To ensure correct interpolation, the phase information is estimated across at least two subsequent pilots. Hence, a minimum filter length of 65 taps. 

Although using blind phase recovery on the data symbols could enhance the recovery metrics, the results presented herein can be viewed as a conservative estimate of the overall performance. Moreover, the phase noise component was modelled to produce approximately the same RPN remainder as used for the corresponding GS optimisation. 

% GMI verification with FEC
In order to validate the GMI-based optimization, we implemented a single-bit extended Hamming code (128,120) with rate $\approx$ 0.94, similar to the one recommended in \cite{oif}. In the 400ZR agreement the Hamming code is used as an inner SD code (in combination with an outer staircase code) with a target post-FEC BER of $4.5\cdot 10^{-3}$. The FEC decoder was a Chase3 SD algorithm \cite{Chase1972} based on the channel bit-wise reliabilities (log-likelihood ratios). Moreover, an ideal random interleaver was adopted to decorrelate bit errors within each received symbol. Although GMI is not necessarily a good indicator for the performance of the Hamming code, at high rates GMI gains are still expected to translate well in terms of post-Hamming FEC BER gains. The latter gains are ultimately the relevant ones for a 400ZR-based system.




==> tools/README <==

August 26, 2015


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.

 2. The \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later.

 3. The \IEEEnoauxwrite command.

 4. The IEEE itemize, enumerate and description list environments.

 5. The complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

 6. The \IEEEQEDhere and \IEEEQEDhereams commands to provide amsthm.sty
    \qedhere functionality to IEEEproof. \IEEEQEDhere is for simple use
    "right on the spot" such as within an IEEEeqnarry:

    \begin{IEEEproof}
       \begin{IEEEeqnarray}{rCl+x*}
        x & = & y & \nonumber\IEEEQEDhere
       \end{IEEEeqnarray}
    \end{IEEEproof}

    While \IEEEQEDhereams is like amsthm's venerable \qedhere and is
    for use within the standard equation environment:

    \begin{IEEEproof}
     \begin{equation}
       x = y \nonumber\IEEEQEDhereams\quad
     \end{equation}
    \end{IEEEproof}

    Note that the qedhere style is normally not done with IEEE-related
    work so these are undocumented features of IEEEtran.cls.

    Thanks Mark D. Butala, Hennadiy Leontyev and Stefan M. Moser for
    suggesting this feature.



IEEEtrantools.sty is not needed and should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
2015/08/26 V1.5 (V1.8b of IEEEtran.cls) changes:

 1) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 2) Fix bug with IEEEeqnarray equation number foreground color
    under the color environment of Beamer class.
    Thanks to Joschi Brauchle for reporting this problem.

 3) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.



********************************** Files **********************************

README                - This file.

changelog.txt         - The revision history.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************


